Deep Reinforcement Learning for Human-Like Driving Policies in Collision Avoidance Tasks of Self-Driving Cars

The technological and scientific challenges involved in the development of autonomous vehicles (AVs) are currently of primary interest for many automobile companies and research labs. However, human-controlled vehicles are likely to remain on the roads for several decades to come and may share with AVs the traffic environments of the future. In such mixed environments, AVs should deploy human-like driving policies and negotiation skills to enable smooth traffic flow. To generate automated human-like driving policies, we introduce a model-free, deep reinforcement learning approach to imitate an experienced human driver's behavior. We study a static obstacle avoidance task on a two-lane highway road in simulation (Unity). Our control algorithm receives a stochastic feedback signal from two sources: a model-driven part, encoding simple driving rules, such as lane-keeping and speed control, and a stochastic, data-driven part, incorporating human expert knowledge from driving data. To assess the similarity between machine and human driving, we model distributions of track position and speed as Gaussian processes. We demonstrate that our approach leads to human-like driving policies.

==> networks_visualization/alphas.tex <==



%\pagestyle{empty}

\def\layersep{2.5cm}
\def\outputdim{3}
\def\hiddenlayerdim{6}
\def\inputlayerdim{5}


\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,\inputlayerdim}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left:] (I-\name) at (0,-\y) {};

    % Draw the first hidden layer nodes
    \foreach \name / \y in {1,...,\hiddenlayerdim}
        \path[yshift=0.5cm]
            node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};
    
    % Draw the second hidden layer nodes
    \foreach \name / \y in {1,...,\hiddenlayerdim}
        \path[yshift=0.5cm]
            node[hidden neuron] (H2-\name) at (\layersep*2,-\y cm) {};

    % Draw the output layer node
    \foreach \name / \y in {1,...,\outputdim}
        \path[yshift=0.5cm]
            node[output neuron,pin={[pin edge={->}]right:}] (O1-\name) at (\layersep*3,-\y cm-1cm) {$\alpha_\y$};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,\inputlayerdim}
        \foreach \dest in {1,...,\hiddenlayerdim}
            \path (I-\source) edge (H1-\dest);

    % Connect every node in the 1st hidden layer with every node in  % the second hidden layer. 
    \foreach \source in {1,...,\hiddenlayerdim}
        \foreach \dest in {1,...,\hiddenlayerdim}
            \path (H1-\source) edge (H2-\dest);
            
    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,\hiddenlayerdim}
        \foreach \dest in {1,...,\outputdim}
            \path (H2-\source) edge (O1-\dest);

    % Annotate the layers
    \node[annot,above of=H1-1, node distance=1cm] (h1-1) {Hidden layer};
    \node[annot,left of=h1-1] {Input layer};
    \node[annot,right of=h1-1](h2-1) {Hidden layer};
    \node[annot,right of=h2-1] {Output layer};
    
    \node[annot,below of=H1-6, node distance=1cm] (h1-6) {600 units};
    \node[annot,left of=h1-6] {300 units};
    \node[annot,right of=h1-6](h2-6) {600 units};
    \node[annot,right of=h2-6] {3 units};


\end{tikzpicture}

==> networks_visualization/ann_architecture_example.tex <==



%\pagestyle{empty}

\def\layersep{2.0cm}
\def\outputdim{2}
\def\hiddenlayerdim{4}
\def\inputlayerdim{3}

\begin{center}
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,\inputlayerdim}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left:] (I-\name) at (0,-\y) {};

    % Draw the first hidden layer nodes
    \foreach \name / \y in {1,...,\hiddenlayerdim}
        \path[yshift=0.5cm]
            node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};
    
    % Draw the second hidden layer nodes
    \foreach \name / \y in {1,...,\hiddenlayerdim}
        \path[yshift=0.5cm]
            node[hidden neuron] (H2-\name) at (\layersep*2,-\y cm) {};

    % Draw the output layer node
    \foreach \name / \y in {1,...,\outputdim}
        \path[yshift=0.5cm]
            node[output neuron,pin={[pin edge={->}]right:}] (O1-\name) at (\layersep*3,-\y cm-1cm) {};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,\inputlayerdim}
        \foreach \dest in {1,...,\hiddenlayerdim}
            \path (I-\source) edge (H1-\dest);

    % Connect every node in the 1st hidden layer with every node in  % the second hidden layer. 
    \foreach \source in {1,...,\hiddenlayerdim}
        \foreach \dest in {1,...,\hiddenlayerdim}
            \path (H1-\source) edge (H2-\dest);
            
    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,\hiddenlayerdim}
        \foreach \dest in {1,...,\outputdim}
            \path (H2-\source) edge (O1-\dest);

    % Annotate the layers
    \node[annot,above of=H1-1, node distance=1cm] (h1-1) {Hidden layer};
    \node[annot,left of=h1-1] {Input layer};
    \node[annot,right of=h1-1](h2-1) {Hidden layer};
    \node[annot,right of=h2-1] {Output layer};
    
    \node[annot,below of=H1-4, node distance=1cm] (h1-4) {4 units};
    \node[annot,left of=h1-4] {3 units};
    \node[annot,right of=h1-4](h2-4) {4 units};
    \node[annot,right of=h2-4] {2 units};


\end{tikzpicture}
\end{center}

==> networks_visualization/critic.tex <==



%\pagestyle{empty}

\def\layersep{2.5cm}
\def\halfoutputdim{6}
\def\hiddenlayerdim{6}
\def\inputlayerdim{5}


\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,\inputlayerdim}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left:] (I-\name) at (0,-\y) {};

    % Draw the first hidden layer nodes
    \foreach \name / \y in {1,...,\hiddenlayerdim}
        \path[yshift=0.5cm]
            node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};
    
    % Draw the second hidden layer nodes
    \foreach \name / \y in {1,...,\hiddenlayerdim}
        \path[yshift=0.5cm]
            node[hidden neuron] (H2-\name) at (\layersep*2,-\y cm) {};

    % Draw the output layer node
    \node[output neuron,pin={[pin edge={->}]right:Output}, right of=H2-3] (O) {$Q$};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,\inputlayerdim}
        \foreach \dest in {1,...,\hiddenlayerdim}
            \path (I-\source) edge (H1-\dest);

    % Connect every node in the 1st hidden layer with every node in  % the second hidden layer. 
    \foreach \source in {1,...,\hiddenlayerdim}
        \foreach \dest in {1,...,\hiddenlayerdim}
            \path (H1-\source) edge (H2-\dest);
            
    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,\hiddenlayerdim}
        \path (H2-\source) edge (O);

    % Annotate the layers
    \node[annot,above of=H1-1, node distance=1cm] (h1-1) {Hidden layer};
    \node[annot,left of=h1-1] {Input layer};
    \node[annot,right of=h1-1](h2-1) {Hidden layer};
    \node[annot,right of=h2-1] {Output layer};
    
    \node[annot,below of=H1-6, node distance=1cm] (h1-6) {600 units};
    \node[annot,left of=h1-6] {300 units};
    \node[annot,right of=h1-6](h2-6) {600 units};
    \node[annot,right of=h2-6] {1 unit};


\end{tikzpicture}

==> sections/discussion_future_work.tex <==

In this paper, we introduced a novel approach to imitate the behavior of an expert driver. For this purpose we have built a full driving simulator environment in Unity. We have focused on a rather simple use-case in which static obstacles were distributed arbitrarily on a two-lane road. We have collected driving data from four participants (experienced drivers) and chose one as a representative expert driver assuming that this expert performs nearly-optimal.

The discussion section is organized as follows. First, the method used in this study will be compared with other commonly used methods with special focus of the benefits of the method selected in this work. Next, the findings of this study will be discussed with respect to the existing literature and the limitations of this work will be discussed. Ultimately, in light of the limitations of the current study, future research directions will be proposed.

In \cite{mombaur2010human}, the authors presented an inverse optimal control (or synonymously known as inverse RL (IRL)) approach to transfer human motions to a humanoid robot. Also, in \cite{ziebart2009human}, the authors suggested an IRL approach to imitate human behavior for route preferences.

While IRL can be used to reproduce human driving behavior distribution based on expert demonstration, our suggested approach allows building a model that incorporates expert demonstrations and basic driving rules (models) in the same approach. We therefore chose an RL approach instead of IRL, which only uses expert demonstrations. For example, if the expert human driver would repeat the same mistake, i.e., provide bad demonstrations, that would be transferred to the agent in IRL. In our RL approach, unwanted driving behavior can be mitigated by increasing the weights of the desired models.
In addition, in IRL we can not become better than the expert whereas in RL, there is a possibility that the agent gets ``better'' than the human expert providing another advantage of the latter approach. Our RL approach also avoids modeling mathematically complex human driving behavior.

In our work, a deep reinforcement learning (DRL) algorithm has been used to model machine driving. We chose Proximal Policy Optimization (PPO) as our learning algorithm, which is a state-of-the-art, on-policy and model-free DRL algorithm. We used Gaussian Processes (GPs) to model and analyze human and machine driving behavior. A stochastic reward function, including expert demonstrations and basic driving behavior, was used to recover the first and second moment of the expert driving distribution. The PPO algorithm was augmented by a Mixture Density Network (MDN) to 
generate more flexible stochastic policies for machine driving .To assess human driving behavior two measurements variables were analyzed: track position and speed.

Two reward functions were introduced - a deterministic and a stochastic one. The first was used to reproduce the mean track position and speed of the expert, while the second was used to recover the mean and variance.

In the determinsitic case the reward function incorporates the mean driving performance provided by the mean of track position and speed as represented by the corresponding GPs models. PPO was implemented with a single multivariate unimodal Gaussian to represent the policy

In the stochastic case the reward function incorporates the mean and variability of track position and speed as represented by the corresponding GPs models. PPO was implemented with a MDN architecture to represent the policy as a mixture of Gaussians.

To the best of our knowledge, this work utilizes a novel, model-free approach, to reproduce a human driving distribution in terms of the mean and the variability (the first and the second moments). We have shown that our method can roughly reproduce the expert driver's driving performance distribution in a complex environment with a high dimensional state space. Track position was better reproduced than speed in both cases. Consistent with our findings, other studies in different domains report similar patterns. In Mombauer et al (\cite{mombaur2010human}), for example, the authors conisdered an IRL problem and reported better results in reproducing a humanoid first moment of position rather than speed. There is one study that was able to report good reproduction of position and speed \cite{lu2018learning}. Nevertheless, this study used a model-based approach rather than a model-free approach that was used in our study.

Dealing with the inherent uncertainty in observed behavior is a major challenge in machine learning. One of the sources of this uncertainty is that the expert's decisions may be based on additional information that is not available to the agent (partially observed environment) \cite{ziebart2009human}. We believe that the features in the state-space provide sufficient information (shown in Table \ref{table:state_and_action}) to the agent to reproduce the track position of the expert driver. In contrast, these features do not provide the agent sufficient information regarding the expert driver's selections of driving speed.

For instance, looking at Figure \ref{fig:speed_limiting_case} panels (a) and (b), there are two straight road sections before the curve that are free of obstacles. The agent identifies these two sections as identical. The human driver, on the other hand, can observe the obstacles after the curve in panel (a) but not in panel (b), and thus, perceives these two road parts as different. In fact, this example emphasizes the flexibility of the human driver to rely on previous knowledge and take into account obstacles that are currently not in the immediate surroundings of the vehicle. The behavior of the automated agent is limited by its sensors and predefined algorithms (e.g., a visual field of view of 300 meters).

As long as we do not provide the agent with additional information (as suggested later in this chapter) to allow it to distinguish between these two road segments, it will probably choose to drive at the same speed.

Also, one can see that the speed was reproduced slightly better for the second case (using the MDN architecture). We believe that here, too, the main reason is that the environment is partially-observed. Following the previous example, the agent identifies two road sections as identical, though they are not. The agent then receives different rewards while expecting to receive the same reward. Therefore, the agent will perceive the environment as stochastic (although it is not from the expert driver's point of view). Namely, we believe that the primary reason for the agent to reproduce the speed better in the second case is the stochasticity of the environment, where the Mixture Density Networks architecture is known to perform better.
\newline
\newline
%%%%% further work and study limitation %%%%
\noindent
Although our approach was able to recover reasonably well  the first and second moments of  track position and to some extend first and second moment of speed in a static obstacle avoidance task, it still has several limitations.

First, in the current setup, the agent fails to recover the exact driving distribution of the expert driver. The model-free approach in a partially observed environment can be restrictive when trying to reproduce the exact expert's distribution. We believe that a richer representation of the state-space may have resulted in a better recovery of the expert driver's driving performance. Specifically, a richer state-space may contain important latent variables that can help the agent to infer the human driver's intent. For example, Convolutional neural networks (CNN) can be used to incorporate camera images along with low sensory data to extract more details (e.g., better road curvature representation, presence of obstacle outside the radar sensor field of view) about the environment. In addition, dealing with a sequential process (as given in our problem), observations are highly correlated meaning that previous observations may affect a driver's behavior in subsequent observations. Thus, one should consider modeling these subsequent observations as dependent. RNN approaches could be used to model the relationship between observations, as they are known for their ability to function better in partially observed environments. 

Second, single use-case optimization, i.e., one track with several static obstacles, brings into question the ability of the agent to generalize and deal with different scenarios, such as different obstacle configurations, dynamic obstacles or extreme cases such as a full blocking of both lanes. Generalization in RL is a challenging problem. In \cite{cobbe2018quantifying} the authors propose to train an agent with diverse situations to improve generalization. Their approach was successfully demonstrated with a relatively simple video game. It took the agent about $10^4$ different levels to acquire a reasonable generalization performance. We believe that training the agent in different obstacle configurations and different tracks can improve its generalization performance.

Third, one should consider using other types of latent variable models instead of MDN that was used in this work, to represent more complex policy models. There are other latent variables models, in contrast to MDNs, that do not need an a priori specification of the number of Gaussians that will be used. By that, they can approximate very complex functions, which is often difficult when the policy is limited to a predefined number of Gaussian. Latent variable models are commonly used in studies dealing with imitation learning.

This work can be extended to deal with scenarios that involve dynamic obstacles, such as other cars, motorcycles or pedestrians. We believe that in such cases relative measurements should be taken into account, for instance, time to collision (TTC), relative distances, and relative speed from different obstacles, as opposed to the case of static obstacles we presented in this work.




==> sections/introduction.tex <==
The 21st century will be the age of autonomous vehicles (AV). This technological revolution will have major impact on our economies, environments and societies and will provide solutions to existing global problems. To enable this technology, many technical challenges have to be resolved. From an algorithmic perspective the two most important are: \textit{perception}, i.e., the understanding of the surrounding environment of the car (e.g. traffic signs, pedestrians, obstacles, vehicles) and the \textit{driving-policy}, i.e., the decision-making process that aims to replace the human driver.

While significant progress has been made to solve the perception problem (e.g., Mobileye), the focus of attention lies now in identifying the correct driving policy, i.e., the question of how the car should act in a multitude of environments and under a multitude of conditions. The success of this challenge will  eventually decide whether self-driving cars will be feasible or not.

Programming an AV behavior is not a trivial task. Traditionally, many solutions use machine learning (ML) approach, since manually defining a set of rules for the car to follow, such as ``Stop if you see red light'', for all complex decision-making scenarios in driving is almost impossible.  Currently, the standard methods used for the control of an AV is a mixture of data-driven and rule-based approaches, where driving commands (steering, gas, and braking)  are obtained and learned from prior knowledge and human data using cameras, sensors, LIDAR, RADAR, and HD-maps.

One of the earliest demonstrations of autonomous driving goes back to 1988 in the study of Pomerleau ``Autonomous land vehicle in a neural network'' or ALVINN \cite{pomerleau1989alvinn}. ALVINN used a fully-connected neural network (NN) with 1,217 units for cameras input, one hidden layer of 29 units, and 46 units output in order to autonomously navigate the car across the North American continent. The NN mapped cameras images to a discrete action space output of 45 units in order to control car steering and one output unit to represent the road intensity for better distinguishing the non-road. Whereas these early studies focused on simple use-cases and environments,  today's autonomous vehicles are tested in much more challenging traffic environments, which are dynamic, stochastic and partially observable. This complexity brought with it the necessity to develop better perception and control capabilities. 

In 2004, the first DARPA Grand Challenge competition was held. Fifteen autonomous vehicles were challenged to travel a 229 km course, starting from Barstow, California to Primm, Nevada. None of the competitors were even close to the finish line. The furthest distance traveled was 12 km \cite{buehler2009darpa}.

One of the breakthroughs in the autonomous-driving field happened a few years later - in the DARPA Urban Challenge in 2007. The challenge called for autonomous-vehicle to drive 97 km through an urban environment interacting with other moving vehicles and obeying the California Driver Handbook.

Much progress has been made in recent years towards autonomous driving. However, a level where a fully autonomous vehicle can travel roads, has not yet been achieved. Many scenarios and environments  are still too challenging for an autonomous vehicle to handle, in contrast to a human driver. Thus, the central question is how can a machine learn from human driving to develop human driving skills, while still encoding basic driving rules that cannot be overwritten. There are good reasons to aim for human-like policies in self-driving cars. First, machine driving can be effective, for example,  in terms of fuel consumption or time, but may show  uncomfortable behavior such as sudden stops, carelessness, or over-caution, which induces discomfort in human passengers. Thus, human factors need to be taken into considerations. Second, autonomous vehicles and conventional cars will share the same traffic environments in the near future, and thus, human drivers need to anticpate the behavior of autonomous vehicles. Adapation will be facilitated if the autonomous vehicle shows human-like driving behavior.

Deep neural networks (DNNs) are considered to be the current workhorse that enable vehicles to learn how to navigate using large amounts of data. While common approaches to find a suitable driving-policy is mainly relying on supervised learning (SL) methods, our work focuses on imitation learning (IL) i.e., learning of the desired behavior by imitating expert behavior. Our purpose is to find human-like policies in static collision-avoidance task of self-driving cars. In order to address such a problem, we are using IL in the context of a deep reinforcement learning (DRL) paradigm. 

In this paper we provide a model-free approach, to reproduce a human driving distribution in terms of the mean and the variability (the first and the second moments). The resulting method utilizes a small amount of human driving data and is relatively easy to implement. In addition, unlike similar approaches such as \textit{inverse reinforcement learning}, the reward function is constructed from human driving data and basic driving rules.

%Our research focused on a rather simple use-case of a two-lane highway where static obstacles (barricades) were arbitrarily distributed along the road (see figure \ref{fig:simulator_env}). Our purpose is to find a driving-policy that matches an experienced human driving-behavior. Eventually, the trained AV should maneuver between the obstacles like an expert human driver in terms of traveling speed and track position.
\begin{figure*}[ht]
    \centering
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/sim1.png}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/sim2.png}
    \end{minipage}
    \caption{Two-lane high-way road. Static obstacles are placed along the road.}
    \label{fig:simulator_env}
\end{figure*}

%We will use a driving simulator, which we developed in Unity, for expert data acquisition and evaluation. The data will be collected from human participants. Gaussian Processes will be used to model the expert driving behavior for two basic metrics (speed and track position). 

%To assess whether the machine develops human-like policies, we will compare the statistic between machine and human driving.

%A state-of-the-art deep reinforcement learning algorithm (Proximal Policy Optimization (PPO)) will be used as the learning algorithm.



==> sections/methods.tex <==




Traditionally, a complete AV system consists of different modules, where each has different responsibilities. The connection of these modules ultimately defines the decision-making process of an AV from sensing, planning to execution. Since our study focuses on finding the driving-policy, we assume that all sensory information is given and processed directly in the driving-simulator. We train a DRL agent directly from low-dimensional observations (e.g. speed, heading angle, track position.) to find the optimal policy and control the car's input commands i.e., steering and throttle, without separation into the different modules. This approach has been successfully demonstrated in the TORCS racing simulator by \cite{koutnik2014evolving, lillicrap2015continuous}.

We will start by describing the simulator environment that we have implemented, the road structure, the use-case, and the state and action space. Section \ref{sec:data_acquisition} describes the ways we used to collect experienced drivers' data. Gaussian processes to model experienced human driving are discussed in Section \ref{sec:modeling_human_behavior}. The proposed reward functions will be discussed in Section \ref{sec:reward_functions}. Finally, the learning algorithm (PPO) will be presented in Section \ref{sec:learning_algorithem}.

\subsection{Simulator Environment}
\label{sec:simulator_env}

A flexible driving-simulator that allows creating different scenarios, road structures, and other objects, such as obstacles, is provided by Unity, a professional game engine written in C\#. Unity is equipped with a Python interface and all algorithms were written in Python. 

A Logitech G29 Driving Force steering wheel and pedals was used in order to manually control the car and to collect data from experienced drivers, as will be described in Section \ref{sec:data_acquisition}.

\subsubsection{Road Structure and Use Case}
\label{sec:road_structure_use_case}
The road  to train the agent consisted of two lanes (3 meters width each) and had a length  of approximately 4.7 km. The road is defined by a closed loop and characterized by straight and curved sections. The road structure is shown in Figure \ref{fig:road_structure}.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{pictures/road_structure.png}
    \end{minipage}
    \caption{The geometry of the road used in the simulation. The road (length 4.7 km, two lanes) consisted of straight and curved segments}.
    \label{fig:road_structure}
\end{figure}

\noindent
Seventeen obstacles (barricades) were placed along the lanes, nine on the right lane and eighth on the left lane, as shown in Figure \ref{fig:simulator_env}.

\subsubsection{State and Action Space}
Table \ref{table:state_and_action} presents the state and the action spaces of the environment, which are both continuous. The torque defines the brake or gas input to the engine, where negative values represent braking input and positive values acceleration input. This definition guarantees that the engine's torque input will not include gas and brake at the same time.
We set the maximum speed of the vehicle to $100 \frac{km}{h}$. A description of the observation ($ob$) variable is shown in figure \ref{fig:ob_sensor}. The different components of the observation have different physical units (for example, speed versus heading). As this may harm the learning process of the networks, we manually scaled all variables between two ranges: $(-1, 1)$ and $(0,1)$, depending on whether the variable can take negative values or not.
\begin{table*}[ht]
\caption{State and Action spaces table of notation. The top of the table displays the state space variables, where each state consists of two subsequent observations (except for $ob$) in order to infer temporal information. The bottom of the table displays the variables of the action space. *$D$ measurement is illustrated in Figure \ref{fig:trackPos}}
\begin{center}
%\centering
\begin{tabular}{ |c||l|c|c|  }
\hline
\multicolumn{4}{|c|}{State Space Variables} \\
\hline
Notation & Description & Range & Scale\\
\hline
$\psi$       & steering & $[-25\degree, 25\degree]$ & $[-1,1]$ \\
$\tau$       & torque: brake + gas & $[-1,1]$ & $[-1,1]$ \\
$V$          & speed & $[0, 100]\frac{km}{h}$ & $[0,1]$ \\
$\theta$     & heading & $[-\pi, \pi]rad$ & $[-1,1]$ \\
$D$          & distance to the dashed line* & $[-6,6]m$ & $[-1,1]$ \\
$D_r$        & distance to the right lane & $[-9,3]m$ & $[-1,\frac{1}{3}]$ \\
$D_l$        & distance to the left lane & $[-3,9]m$ & $[-\frac{1}{3},1]$ \\
$\delta_{fr}$  & nearest front obstacle in the right lane & $[0,300]m$ & $[0,1]$ \\
$\delta_{fl}$  & nearest front obstacle in the left lane & $[0,300]m$ & $[0,1]$ \\
$\delta_{br}$  & nearest back obstacle in the right lane & $[0,300]m$ & $[0,1]$ \\
$\delta_{bl}$  & nearest back obstacle in the left lane & $[0,300]m$ & $[0,1]$ \\
\textit{ob}  & 288 obstacles and road boundaries sensors & $[0,300]m$ & $[0,1]$ \\
\hline
\multicolumn{4}{|c|}{Action Space Variables} \\
\hline
$\psi$       & steering & $[-25\degree, 25\degree]$ & $[-1,1]$ \\
$\tau$       & torque: brake + gas & $[-1,1]$ & $[-1,1]$ \\
\hline
\end{tabular}
\label{table:state_and_action}
\end{center}
\end{table*}

The state-space has 310 dimensions and is defined by two subsequent observations (except for $ob$). The subsequent observations have significantly improved the performance of the algorithm and the training time. When exceeding road boundaries, the values of $ob$ sensors are not reliable and are set to $-1$.
The action space has two dimensions consisting of steering and braking/gas commands.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{pictures/ob_sensor.png}
    \caption{The distance sensor providing the observation measurement $ob$. The sensor range is set to a field of view of $360\degree$ and a radius of $300$ meters. This range is covered by 288 equally separated rays. Each ray determines the distance from the vehicle to the nearest road obstacle or road boundary.}
    \label{fig:ob_sensor}
\end{figure}

\subsection{Human Driving Data Acquisition}
\label{sec:data_acquisition}
To collect data from human experienced drivers, we performed an experiment with 4 participants.
Each of the participants repeatedly traveled the road for eight rounds while providing gas, braking and steering controls. The participants were instructed to drive as they would normally drive in similar real-world situations except for the following additional instructions: (1) maintain driving on the right lane unless you overtake a vehicle, (2) maintain a speed limit of 100 km/h.

Each participant drove two practice rounds to get familiar with the simulated environment. During the experiment, the data - presented in the table of content \ref{table:state_and_action} - were collected together with the global world coordinates\footnote{The global world coordinates were used to calculate the travel distance by accumulating the Euclidean distance of each pair of subsequent points $\sqrt{(x_1-x_2)^2+(y_1-y_2)^2}$ for each round.} $(x,y,z)$. The sampling rate was 10 Hz.

Throughout the experiment, we noticed that two of the participants were struggling to keep the car in the lane, and their driving seemed to be unstable with high fluctuations. Another participant was mostly driving while pressing the gas pedal to the end and reaching to a constant speed of $100$ km/h. After slowing down, the participant aggressively accelerated until the car slowed  its acceleration sharply as a result of the speed limit. As this was a rather unnatural driving style, we decided to exclude these data. We selected one participant who demonstrated good driving skills to represent the desirable human driving behavior. From now on, we will refer to this participant as the ``expert driver'', as it is commonly termed in imitation learning literature notations.

\subsection{Modeling Human Driving Behavior}
\label{sec:modeling_human_behavior}

Modeling human driving behavior is a difficult task due to the many factors that affect driving, such as the road environment, other traffic participants, traffic rules, driver intention and internal driver states, just to name a few \cite{leung2016distributional}. There is a large amount of literature about building mathematical models for various aspects of driving \cite{borrelli2005mpc, kong2015kinematic}. Generally, driving is defined by  an environment, which is  stochastic, dynamic and partially observable, and therefore, poses big challenges to any modeling approach. 
In a reinforcement learning modeling approach, which we intend to apply, this implies to engineering a presumably complicated reward function. To facilitate the reward engineering process we decompose our reward function into two parts: a model-driven part and a data-driven part. The model-based part enforces basic driving rules, such as staying within the road boundaries and speed limits, whereas the other part incorporates knowledge of expert driver in the form of experimental data.

However, hand-crafting such a reward function in a high-dimensional and non-linearity feature space, along with a stochastic driving behavior of the human driver, could be a hard task. This fact motivated us to use Gaussian processes (GPs).

A GP allows to model a distribution over functions, which then can be sampled. We chose one of the participants as a representative expert driver for the reasons explained in Section \ref{sec:data_acquisition}. Based on the expert driver data that we recorded from the simulator, as described in Section \ref{sec:data_acquisition}, we used GPs in order to model the distributions over two measurement variables: track-position ($D$) and speed ($V$). In the remaining Section, we model the distributions of the variables using GPs and show how to sample from them.

We found the \textit{Rational Quadratic kernel} to be the best fit, as it was able to approximate a function that best represents the data. The independent variable was defined by the traveled Euclidean distance (arc-length). The noise parameter in the GP was tuned such that the demonstrated trajectories of the expert driver will be properly covered inside a 99\% confidence interval of the GPs.

\subsubsection{Track Position}
The track-position $D$ refers to the distance between the car and the dashed line, as illustrated in Figure \ref{fig:trackPos}. 

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{pictures/trackPos.png}
    \end{minipage}
    \caption{Illustration of the track position ($D$). The track position is measured with respect to the road's center-line (dashed line), which divides the road into 2 lanes. The track position will take value 3m and -3m when the vehicle is precisely in the middle of the right lane or the left lane, respectively. The extreme values of 6m and -6m correspond to the position of the car on the right and left margin line, respectively.}
    \label{fig:trackPos}
\end{figure}

Figure \ref{fig:GP_trackPos} presents the measured distribution for track position obtained from the expert driver as well as the modeled distribution using GP as a function of traveled distance.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{pictures/expert_trackPos.png}
    \end{minipage}
    \caption{The expert driver distribution of the car track position (red) and the modeled distribution using GP (gray) as  a function of traveled distance. The shaded gray area represents a 99\% confidence interval. The blue line is the mean.}
    \label{fig:GP_trackPos}
\end{figure}

\subsubsection{Speed}
Figure \ref{fig:GP_speed} presents the measured distribution for speed, obtained from the expert driver, as well as the modeled distribution using GP as a function of traveled distance.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{pictures/expert_speed.png}
    \end{minipage}
    \caption{The expert driver distribution of speed (red) and the modeled distribution using GP (gray) as  a function of traveled distance. The shaded gray area represents a 99\% confidence interval. The blue line is the mean.}
    \label{fig:GP_speed}
\end{figure}

It is noticeable that there are significant variations in the velocities provided by the expert driver. This has made it more difficult to approximate the distribution of the speed.

\subsubsection{Trajectory Sampling Process}
\label{sec:traj_sampling}

We are interested in finding the expert driver's stochastic driving behavior. In the following Section \ref{sec:first_and_second_moment}, we will describe how we reproduced the expert driver's distribution by using a stochastic reward function. This reward function is constructed using samples taken from the GPs distributions we presented in Section \ref{sec:modeling_human_behavior}. Thus, in the remaining part of this Section, we will present the sampling process.

After finding the expert driver's probability distribution over the functions of the two basic measurement variables ($D$ and $V$), we randomly sampled 100 trajectories (per dependent measurement) within their bounds of 99\% confidence interval. 
The number of samples is determined by their ability to cover the 99\% confidence interval well. We made sure that the trajectories were within the range by multiple random sampling while rejecting samples that were out of bounds. The process ended when the predetermined number of samples (100) was reached.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.5\textwidth}
    \includegraphics[width=\columnwidth]{pictures/bounded_samples_trackPos.png}
    \caption*{(a)}
    \end{minipage}
    \vfill
    \begin{minipage}[b]{0.5\textwidth}
    \includegraphics[width=\columnwidth]{pictures/bounded_samples_speed.png}
    \caption*{(b)}
    \end{minipage}
    \caption{100 random trajectories sampled from the expert driver's distribution: (a) Shows the samples of the track position $D$ metric. (b) Shows the samples of the speed $V$ metric. Each sample is within the bounds of 99\% confidence interval. The dashed lines represent the samples, and the solid blue line represents the mean.}
    \label{fig:bounded_samples_GPs}
\end{figure}


\section{Reward Functions}
\label{sec:reward_functions}

In this section, we will propose two reward functions. The first reward function is deterministic and capable of reproducing the mean of the expert driver's probability distribution of track position and speed. The second one is stochastic and used to recover the first and also the second moment (variance) of the expert driver's probability distribution of track position and speed.

\subsubsection{First Moment (Mean)}

We first aimed to find a driving policy that reproduces the expert driver's mean driving behavior. We considered the following deterministic reward function:
\begin{equation}
R(s_t,a_t) = 
\begin{cases}\!% alignment adjustment
\begin{aligned}[b]% adjust case condition placement here, use [t]op, [b]ottom, or [c]enter (default)
\overline{V}_h - |\overline{V}_h - V_a |\bigg|_t - c_1 {|\overline{D}_h - D_a|}\bigg|_t \\-c_2 |\psi_t - \psi_{t-1}| - c_3|\tau_t - \tau_{t-1}|
\end{aligned}
\\
-100\,, \; \mbox{if}\; s_t = s_T
\end{cases}\,,
\label{eq:deterministic_reward_function}
\end{equation}
where $s_T$ are termination states defined by 
$s_T$ = \{exceeding road boundaries, driving slower than 5 km/h, driving in the opposite direction\}.
\newline
\newline
In Table \ref{table:reward_notation} we provide all variables and parameters, which determine the reward function. Speed $V$ and track position $D$ were not scaled while the steering command $\psi$ was scaled to the range [-1,1].
\begin{table}[H]
\caption{Variables and parameters that determine the reward function.}
\begin{center}
\begin{tabular}{ |c||l| }
\hline
Notation & Description \\
\hline
$a$                 & agent \\
$h$                 & human \\
$V$                 & speed \\
$D$                 & track position \\
$\psi$              & steering \\
$\tau$              & torque: brake + gas \\
$c_1$               & penalty weight for lane position deviation \\
$c_2$               & penalty weight for steering oscillation \\
$c_2$               & penalty weight for torque oscillation \\
\hline
\end{tabular}
\label{table:reward_notation}
\end{center}
\end{table}
We will discuss next each term in the reward function (\ref{eq:deterministic_reward_function}). The first term in (\ref{eq:term_1}) incorporates the mean of the speed of the human expert driver, $ \overline{V}_h$, as well as the current speed of the agent $V_a$:
\begin{equation}
\overline{V}_h - | \overline{V}_h-V_a| \bigg|_t \,.
\label{eq:term_1}
\end{equation}

The agent gets a higher reward when driving as close as possible to the mean of the human speed w.r.t the traveled distance at timestep $t$. This term may be either positive ($0<V_a< 2\overline{V}_h$)  or negative ($V_a > 2\overline{V}_h)$. The agent can get a maximum reward of
\begin{equation}
\overline{V}_h\bigg|_t \,,
\label{eq:max_reward_term_1}
\end{equation}

\noindent
if there is no deviation of the agent's speed from the mean human speed.

The second term in (\ref{eq:term_2}) defines the deviation of the agent from the mean track position of the human expert driver and the agent:
\begin{equation}
c_1 {|\overline{D}_h - D_a|}\bigg|_t\,,
\label{eq:term_2}
\end{equation}
where $c1$ is a penalization weight that was set to 20. The minimum penalty is zero, and the maximum penalty is:
\begin{equation}
c_1 \cdot 12\,,
\label{eq:term_2_max_penalty}
\end{equation}
where the value 12 represents two lane widths. The third and the forth term are smoothing terms for steering and torque commands, respectively, and do not incorporate any human data. $c2$ and $c3$ are penalization weights that were set to 100, and 10 respectively.

\subsubsection{First and Second Moments (Mean and Variability)}
\label{sec:first_and_second_moment}
The previous reward function was constructed to capture the mean expert driver's driving behavior. In this section we are aiming to find a reward function that can recover the mean of the expert driver's driving behavior as well as it its variance. For this purpose we have define a stochastic reward function using GPs. It is important to emphasize that in this approach we are not using any underlying dynamic model, but are operating in a purely model-free framework.

After off-line sampling from the expert driver's distributions (as shown in section \ref{sec:traj_sampling}), in each episode, we randomly choose a different sample to determine the reward function.

That is to say, the reward function is stochastic\footnote{Due to computational limitation, we took a large number of samples (100) that were sufficient to capture the distribution within the range of a 99\% confidence interval (as presented in Section \ref{sec:modeling_human_behavior}). With enough computational power, one can try using on-line sampling.} and defined as follows: 

\begin{equation}
R^j(s_t,a_t) = 
\begin{cases}\! 
\begin{aligned}[b]
(V^j_h - |V^j_h - V_a|)\bigg|_t - c_1 {|D^j_h - D_a|}\bigg|_t \\ -c_2 |\psi_t - \psi_{t-1}| - c_3|\tau_t - \tau_{t-1}|
\end{aligned}
\\
-100\,, \; \mbox{if}\; s_t = s_T 
\end{cases}\,,
\label{eq:stochastic_reward_function}
\end{equation}
where $s_T$ are termination states defined by 
$s_T$ = \{exceeding road boundaries, driving slower than 5 km/h, driving in the opposite direction\}.
\newline
\newline
The notations are similar to the ones presented in Table \ref{table:reward_notation}. However, this reward function differs from the previous one in that the measurement variables were changed from the mean behavior ($\overline{D}_h, \overline{V}_h$) to samples ($D^j_h, V^j_h$), where index $j$ represents sample $j$.

This will ultimately lead to stochastic behavior due to the assignment of different probabilities of choosing actions (recall we run a stochastic policy) within the expert driver's distributions.

\subsection{The Learning Algorithm}
\label{sec:learning_algorithem}
We considered two state-of-the-art deep reinforcement learning algorithms to learn a driving policy: Deep Deterministic Policy Gradient (DDPG) and Proximal Policy Optimization (PPO). Ultimately, we decided to choose PPO as the learning algorithm. Hyperparameters tuning in DDPG turned out to be difficult resulting in unstable behavior. This was observed in spite of trying different hyperparameter settings (such as different weights initialization, number of hidden layers, number of neurons in each layer), and using prioritized experience replay (PER).

In PPO we used generalized advantage estimation (GAE) for computing variance-reduced advantage function. The hyperparameter settings are provided in Table \ref{table:PPO_hyperparameters}.

\subsection{Networks Architecture}

Our objective is to imitate the stochastic behavior of an expert driver while obeying basic driving rules. The goal of reproducing the expert driver's stochastic behavior motivated us to use use a Mixture Density Network with three\footnote{The number of Gaussians was arbitrarily chosen. No attempt was made to adjust this hyperparameter.} Gaussians and covariance matrices to represent the actor policy. We also used a different network to approximate the mixing coefficients for each Gaussian. This approach results in three different networks — one for the critic, second for the actor, and third for the mixing coefficients.

\subsubsection{The Actor Network Architecture}

The actor-network architecture is constructed of an input layer of 300 units, 2 hidden layers of 600 units each\footnote{No significant attempt was made to adjust the number of hidden layers and their units.}, and an output layer of 12 units. We use the ReLU activation function between the different layers except for the output layer, where we use two different activation functions to bound the mean and the variance values, as will be later discussed. The 12 units were divided into 2, where the first 6 units represent the mean values of the Gaussians, and the other 6 units represent the covariance matrices as follows. The first 6 units are divided into 3 pairs (as the chosen number of Gaussians), where each pair consisting of the mean value of steering and throttle commands, $\mu_s$ and $\mu_t$ respectively. The actor-network architecture diagram is illustrated in Figure \ref{fig:actor_net_arch} 
\begin{figure}[ht]
    \resizebox{0.5\textwidth}{!}{
    \centering
    \input{networks_visualization/actor.tex}}
    \caption{The actor-network architecture: Input size with 300 units, two hidden layers with 600 units size each, and an output layer with 12 units. The output layer is divided into three different multivariate  - Gaussians. $\mu_s$ and $\mu_t$ represents the mean values of the steering and the throttle commands, respectively. $\sigma_s$ and $\sigma_t$ represents the variance values of the steering and the throttle commands, respectively.}
    \label{fig:actor_net_arch}
\end{figure}

The first 6 values (of the means) are passed through a SoftSign activation function in order to bound to values between -1 to 1, as the control commands are bounded. The last 6 values (of the covariances) are passed through the following customized activation function:
\begin{equation}
\label{eq:custom_activation_function}
f(x) = \frac{1}{16}\cdot Sigmoid(3x)
\end{equation}

Two reasons led us to construct the customized activation function. First, we would like to have non-negative variance for each of our Gaussian. Second, while a simple Sigmoid activation function meets the first requirement, it results in a relatively large value for the variance ($>0.1$). This led to a disproportionate amount of noise and caused the agent to get stuck in a  local minimum at the very first start. We therefore decided to set an upper-bound of the variance to 1/16.

Form the network output we constructed three diagonal covariance matrices, which are then used along with the mean vectors to construct three different multivariate Gaussians. 

\subsubsection{The Critic Network Architecture}
The critic-network uses the same architecture except for the output layer that now consists only with one neuron output, the Q-value.

A ReLU activation function was used in all layers except for the last layer, where we used a linear activation function.

\subsubsection{The Mixing Coefficients Network Architecture}

Similarly, the mixing coefficient network\footnote{While the mixing coefficients could be included as part of the actor's output layer, no such attempt was made.} has the same architecture as for the actor and critic except that the output layer consists of 3 neuron outputs (as the number of the different Gaussians). We used ReLU-activation function for all layers except for the output layer, which uses a softmax activation function in order to maintain $\sum \limits_{i} \alpha_i = 1$.

\subsection{Exploration Strategy and Update Setup}

One of the challenges in RL is the problem of exploration. PPO, our  learning algorithm in this work, is an on-policy algorithm that trains a stochastic policy. The exploration occurs by sampling actions according to its stochastic policy. Typically, PPO uses a Gaussian (or multivariate Gaussian - depending on the action-space dimensions) as its stochastic policy. The amount of exploration in PPO is affected by both the initial value of the covariance matrix and the training procedure. In the standard settings of a fixed initial state and fixed-length episodes, imitation learning is often unsuccessful. 
 
We used the ideas of \textit{initial state distribution} and \textit{early termination}, as suggested in \cite{peng2018deepmimic}, to improve the exploration.

The \textit{early termination} conditions, as described in the proposed reward functions, as given in (\ref{eq:deterministic_reward_function}, \ref{eq:stochastic_reward_function}) are: exceeding road boundaries, driving slower than 5 km/h, and driving in the opposite direction. As to the \textit{initial state distribution}, we initialized the agent in a different state (in each episode) by required it to reach a certain randomly sampled speed. The initial required speed of the car samples from a uniform distribution between 30 to 90 km/h. Both of these modifications dramatically improved learning time and helped avoid poor local minimums in the early stages of the learning process.
\newline

The high randomness at the beginning causes the agent to terminate after a few small steps of about 30-40. A full round of the track requires about 2000 steps. On the one hand, we want a number of steps that will include at least one full round of the track, so that the policy update process can take the entire track driving into account. On the other hand, we do not want to wait a high number of steps until the policy is updated at the beginning. This led us to define a dynamic batch size that grows with agent performance. The dynamic batch size update is described in the pseudocode of Algorithm \ref{algorithem:dynamic_batch_size_update}.

\input{pseudocodes/dynamic_batch_update.tex}

\noindent
where $\textit{completed rounds}$ is a Boolean variable indicating whether the agent has completed two rounds. The $\textit{remainder}$ variable is a remainder of time-steps that needs to be subtracted from the $\textit{agent's max length}*2$ so that the new batch size $B$ can be equally divided for mini-batches\footnote{A multiplier of $2$ is used, so the batch size is about twice the maximum number of times the agent can execute per episode.}. $B$ and $MB$ were initialized to 512 and 256, respectively.

In addition, an entropy coefficient of 0.005 was added to the objective function in order to ensure sufficient exploration, as suggested in past works \cite{williams1992simple, mnih2016asynchronous}.



==> sections/related_work.tex <==
Many studies have been tried to model the human driving behaviour by learning from demonstrations. Known models based on control theory include model predictive control \cite{qu2014switching}, Markov chain models \cite{zou2016real}, and adaptive control \cite{koh2015integrated}. These methods are typically require a significant amount of prior knowledge to build a reliable model dynamics. The amount of the required prior knowledge is increasing with the task complexity, which sometimes is not practic.

In recent years, mainly as a result of an increase in computing power and technological advances in academia and industry, deep learning has become a popular mechanism for solving different driving tasks. Numerous works have demonstrated robotic control using RL. 

In \cite{lillicrap2015continuous}, have used a deep deterministic policy gradient (DDPG) algorithm to control a car in the simulator environment Torcs \cite{loiacono2013simulated}, in both low-dimensional (sensory data) and high-dimensional (from pixels) state spaces. This work used a reward function, which provides a positive reward at each step for the velocity of the car projected along the track direction and a penalty of $-1$ for collisions. While this work successfully exemplified a highway driving control scenario, it did not deal with human driving behavior.

In \cite{codevilla2018end}, the authors have used a vision-based imitation learning approach to control a car in an urban driving simulator environment (CARLA \cite{dosovitskiy2017carla}) and a realistic simulation.

In \cite{abbeel2004apprenticeship}, the authors present an imitation learning (IL) approach, in which the reward function is unknown and needs to be extracted from the expert demonstrations. This method is known as \textit{inverse reinforcement learning} (IRL) \cite{ng2000algorithms}. Additional constraints need to be imposed in IRL resulting a variety of algorithms. Evaluation for this approach was done in a 2D driving simulator.

Supervised-learning approaches that are used to learn to imitate an expert, known as \textit{behavior-cloning}. In \cite{udacitybehaviorcloning}, a convolutional neural network (CNN) was used to map images as inputs to demonstrated expert actions as outputs. However, behavior-cloning has a know generalization problem that accrues when the agent faces situations it did not experience as part of its training set.

In \cite {lu2018learning}, the authors introduced a human driving behavior control algorithm. They used a combination of offline learning and online learning to alleviate the poor adaptation problem to newly collected driving data. The algorithm was evaluated in a 3D simulation of a complex driving scenario where other cars were traveling on the road. However, no assessment of human behavior variability was conducted.

In this work, we use reinforcement learning (RL) as our algorithmic approach to imitate an experienced driver. We demonstrate human driving behavior in terms of mean and variance (first and second moments). We use offline learning to model the distribution of human behavior based on collected driving data. We use a model-free approach to train the agent to control the car so that it drives more human-like. We focused on the static obstacles collision avoidance task.

==> sections/results.tex <==



In this section we will present our simulation results of applying model-free deep reinforcement learning algorithms to 
transfer expert human driving policies to a learning agent for a static obstacle avoidance task. In Section \ref{sec:recover_mean_behavior} we present our results for recovering the first moment (mean) of the expert distributions using a deterministic reward function, whereas a stochastic reward function is used in Section \ref{sec:recover_mean_and_variability}  to recover the first and second moment (mean and variance).

\subsubsection{Trained Policy - Mean}
\label{sec:recover_mean_behavior}
To reproduce the mean behavior of the expert human driver, we used a deterministic reward function, as given in (\ref{eq:deterministic_reward_function}). When evaluating agent's driving, we let the agent drive in deterministic mode. Namely, we used the mean values from the actor-network output to control the agent without constructing a multivariate Gaussian for sampling. The reason we did this is that we were interested in reproducing the mean (deterministic) behavior. Figure \ref{fig:agent_deterministic_vs_human_dist} shows trajectories (red) for track position and speed of the agent after training as well as GPs that were fitted to data obtained from 7 rounds of agent driving. Shown is the mean (solid lines) and a 99\% confidence interval (shaded area). Because the agent learned the mean behavior of the driver, the variance in the policy is so minimal that the shaded area is hardly visible.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/agent_deterministic_trackPos.png}
    \caption*{(a)}
    \end{minipage}
    \vfill
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/agent_deterministic_speed.png}
    \caption*{(b)}
    \end{minipage}
    \caption{Seven rounds trajectories of the agent and GP regression: (a) Track position: trajectories are shown in red. The mean of the GP is shown as an orange line and 99\% confidence interval as an orange shaded area. (b) Speed distributions: same as in a.}
    \label{fig:agent_deterministic_vs_human_dist}
\end{figure}

Figure \ref{fig:agent_deterministic_vs_human_dist} shows the comparison of human expert with agent driving.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/agent_deterministic_vs_expert_trackPos.png}
    \caption*{(a)}
    \end{minipage}
    \vfill
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/agent_deterministic_vs_expert_speed.png}
    \caption*{(b)}
    \end{minipage}
    \caption{Comparison between human and expert driving distributions: (a) Track position: The means of the GPs is shown in solid lines and 99\% confidence intervals in shaded areas. (b) Speed: same as in a.}
    \label{fig:agent_deterministic_policy_results}
\end{figure}

One can see that the agent overestimated the speed. We wondered why the agent was having trouble recovering the speed but was able to recover the track location fairly accurately. One reason could be that the agent should be trained for a longer time to recover local minimums. However, we doubt that mainly because we trained the agent for a very long time (about five days) in high dimensional state space. It is known that in a high dimensional space the chance of getting stuck in a local minimum becomes smaller.

Second, using only one Gaussian to represent the actor policy and in a partially-observed environment, we believe the agent was having difficulty in capturing the environment well enough to reproduce the speed. Further explanation will be presented in the discussion chapter.

\subsubsection{Trained Policy - Mean and Variance}
\label{sec:recover_mean_and_variability}
In order to reproduce also the variability of expert human driving, a stochastic reward function, as given in (\ref{eq:stochastic_reward_function}), had to be used. Figure \ref{fig:agent_policy_results} shows GP regression of the agent driving for the two measurements: track position and speed. 
\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/agent_trackPos.png}
    \caption*{(a)}
    \end{minipage}
    \vfill
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/agent_speed.png}
    \caption*{(b)}
    \end{minipage}
    \caption{Seven rounds trajectories of the agent and GP regression: (a) Track position: trajectories are shown in red. The mean of the GP is shown as an orange line and 99\% confidence interval as an orange shaded area. (b) Speed distributions: same as in a.}
    \label{fig:agent_policy_results}
\end{figure}

In an attempt to recover the expert's driving distribution, we expect to see that the agent's distribution overlaps with that of the expert. Figure \ref{fig:agent_vs_human_dist} shown the comparison of the agent and the human driving for the two measurements: track position and speed.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/agent_vs_expert_trackPos.png}
    \caption*{(a)}
    \end{minipage}
    \vfill
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/agent_vs_expert_speed.png}
    \caption*{(b)}
    \end{minipage}
    \caption{Comparison between human and expert driving distributions: (a) Track position: The means of the GPs is shown in solid lines and 99\% confidence intervals in shaded areas. (b) Speed: same as in a.}
    \label{fig:agent_vs_human_dist}
\end{figure}

It is noticeable that the agent failed to recover the speed distribution in some sections along the track. We believe this is to some extent related to an agent acting in a partially observable environment. For example, the field of view of the agent is strictly limited to 300 meters in our simulations, which may be different for a human driver, which may have a larger field of view and  also may store information about obstacles and road structure in memory. We hypothesize that the agent's limited field of view, along with the road structure and the location of the obstacles, all have a significant impact on it decisions regarding the speed of travel. Figure \ref{fig:speed_limiting_case} shows one such case, where both road sections are similar in characteristics but their average travel speed was different. This example is reflected in graph (b) in Figure \ref{fig:agent_vs_human_dist} at a traveled distance of 1,000 meter (X axis). One can notice that after when the agent detected the obstacle, it starts to slow down. In contrast, the expert driver, whose familiar with this road section and except this obstacle, begins to slow down earlier.

\begin{figure}[ht]
    \centering
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/curved_section_1.png}
    \caption*{(a)}
    \end{minipage}
    \vfill
    \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pictures/curved_section_2.png}
    \caption*{(b)}
    \end{minipage}
    \caption{Two road areas that are similar in curvature are shown: (a) Shows a road area where immediately after the turn, there is an obstacle (bounded by a red square), causing the expert to slow down the speed of travel within the curvature section. (b) In contrast, displays a road area where there is no obstacle after turning, allowing the expert to accelerate in the curvy section and travel at high speed. Both (a) and (b) have no obstacles within the agent's field of view. The blue arrow shows the car traveling direction.}
    \label{fig:speed_limiting_case}
\end{figure}

